Modeling Multiphase Flow Through and Around Multiscale Deformable Porous Materials

Detailed understanding of the coupling between fluid flow and solid deformation in porous media is crucial for the development biomedical devices and novel energy technologies relating to a wide range of geological and biological processes. Well established models based on poroelasticity theory exist for describing coupled fluid-solid mechanics. However, these models are not adapted to describe systems with multiple fluid phases or 'hybrid-scale' systems containing both solid-free regions and porous matrices. To address this problem, we present a novel computational fluid dynamics approach based on a unique set of volume-averaged partial differential equations that asymptotically approach the Navier-Stokes Volume-of-Fluid equations in solid-free-regions and Biot's Poroelasticity Theory in porous regions. Unlike existing multiscale multiphase solvers, it can match analytical predictions of capillary, relative permeability, and gravitational effects at both the pore and Darcy scales. Through careful consideration of interfacial dynamics and extensive benchmarking, we show that our model accurately captures the strong two-way coupling that is often exhibited between multiple fluids and deformable porous media during processes such as swelling, compression, and fracturing. The versatility of the approach is illustrated through studies that 1) quantified the effects of microporosity on sedimentary rock permeability, 2) identified the governing non-dimensional parameters that predict capillary and viscous fracturing in porous media, 3) characterised the effects of cracking on hydraulic fracture formation, and 4) described wave absorption and propagation in poroelastic coastal barriers. The approach's open-source numerical implementation 'hybridBiotInterFoam', marks the extension of computational fluid dynamics simulation packages into deformable, multi-phase, multiscale porous systems.

==> chapters_alt/6_PRLApplications.tex <==
%\begin{savequote}[75mm]
%This isn't right. This isn't even wrong.\qauthor{Wolfgang Pauli}
%\end{savequote}
\begin{savequote}[75mm]
The most exciting phrase to hear in science, the one that heralds the most discoveries, is not ‘Eureka!’ but ‘That’s funny…’\qauthor{Isaac Asimov}
\end{savequote}

\chapter{Capillary and Viscous Fracturing During Drainage in Porous Media} \label{chapter:PRL}

\newthought{In this chapter,} we use the Multiphase DBB framework to study the transition from uniform fluid invasion to capillary and viscous fracturing during drainage in porous media. To do so we examine multiphase flow in deformable porous media in a broad range of flow, wettability, and solid rheology conditions. We then demonstrate the existence of two fracturing transitions controlled by two non-dimensional numbers that quantify the balance of viscous, capillary, and structural forces in a porous medium. We then use these parameters to establish a first-of-its-kind phase diagram for material failure caused by multiphase flow in poroplastic media. This chapter is adapted from \citet{Carrillo2021}.

\section{Introduction}

Multiphase flow in deformable porous media is a ubiquitous phenomenon in natural and engineered systems that underlies key processes in water and energy resource engineering and materials science, including membrane filtration, soil wetting/drying, unconventional hydrocarbon recovery, and geologic carbon sequestration \citep{Bacher2019,Rass2018,Towner1987}. A key obstacle to more accurate representations of this phenomenon is our limited understanding of the transition from fluid invasion to flow-induced fracturing, i.e., material failure caused by multiphase flow. In large part, this limitation is caused by a lack of computational approaches capable of representing multiphase flow in fractured deformable porous media. 

The scientific database on \textit{multiphase} flow within \textit{static} porous media is extensive and includes detailed examinations of the influence of wettability, viscosity, and flow rate on flow in unsaturated porous media at multiple scales. In particular, existing studies have demonstrated how capillary forces give rise to differences between drainage and imbibition \citep{Lenormand1986}; how the ratio of fluid viscosities controls the stability of the invading fluid front \cite{JorgenMalby1985,Saffman1958,Stokes1976}; and how the magnitude of the capillary number (i.e. the ratio between viscous and capillary forces) delineates distinct flow regimes \citep{Ferer2004,Yortsos1997}. Each of the aforementioned controls is highly dependent on the system of interest, leading to significant non-linearity that complicates efforts to develop general relative permeability and capillary pressure models \citep{Picchi2018,Picchi2019,RHBrooks1964,VanGenutchen1980}.

Flow of a \textit{single fluid phase} through \textit{deformable} porous media also has been studied in depth. Numerical modeling studies are largely based on the work of Biot and Terzaghi \citep{Biot1941,Terzaghi1943} and have been used to reproduce the behavior of arteries, boreholes, swelling clays, and gels \citep{Auton2017a,Bertrand2016b,Carrillo2019,MacMinn2015a}. In the last decade, fundamental studies have generated detailed information of the dynamics that arise from fluid-solid couplings beyond the ideal poroelastic regime, including fracturing, granular fingering, and frictional fingering \citep{Campbell2017,Sandnes2011a,Zhang2012}. In particular, these studies have shown that the main parameters controlling the deformation of a porous solid by single phase flow are the material softness and the magnitude of the fluid-solid momentum transfer \citep{Sandnes2011a}.

The study of \textit{multiphase} flow in a \textit{deformable} porous medium is inherently more complex than the problems outlined above, as it requires simultaneous consideration of capillarity, wetting dynamics, fluid rheology, and solid deformation. Deformation modes associated with material failure (i.e., fracturing) present a notably arduous challenge as they require simultaneous representation of multiphase flow in fractures and in the surrounding porous matrix. The few existing detailed examinations of this phenomenon have focused exclusively on the grain scale. Notably, Holtzman \& Juanes \citep{Holtzman2010a,Holtzman2012a} used experiments and discrete element models to demonstrate that the transitions between capillary fingering,
viscous fingering, and fracturing during multiphase flow in granular media reflect two non-dimensional numbers: a fracturing number (ratio of fluid
driving force to solid cohesive force) and a modified capillary number (the ratio between viscous and capillary pressure drops). Other discrete element approaches have shown that fracturing is highly dependent on the invading fluid's capillary entry pressure
\citep{Jain2009,Meng2020}.

To the best of our knowledge, no
experimental or numerical investigation has simultaneously explored the effects of flow rate, wettability, and
deformability during multiphase flow in deformable porous media at the \textit{continuum scale} and/or identified the controlling
parameters that relate \textit{all three} properties within a single comprehensive phase diagram. Here, we use simulations carried out with the Multiphase Darcy-Brinkman-Biot (DBB) framework \citep{Carrillo2020MDBB} to fill this knowledge gap and identify non-dimensional parameters that govern multiphase fluid invasion and fracturing in deformable porous media. 

\section{Numerical Simulations}

\subsection{Crossover from Imbibition to Fracturing in a Hele-Shaw Cell } \label{subsect:Huang}

As a starting point, we applied the Multiphase DBB framework to model the crossover between fluid imbibition and fracturing in porous media. Here, the aim is to replicate experiments by \citet{Huang2012a} involving the injection of aqueous glycerin into dry sand at incremental flowrates within a 30 by 30 by 2.5 cm Hele-Shaw cell. As shown in Figs. \ref{fig:hele-shaw} and \ref{fig:Huang_Frac}, these experiments are inherently multiphysics as fluid flow is governed by Stokes flow in the fracture (aperture $\sim$cm) and by multiphase Biot Theory in the porous sand (pore width $\sim 100\mu$m).

Numerical parameters were set to the known properties of aqueous
glycerin, air, and sand (${\rho }_{gly}=1250\ \mathrm{kg/m^3}$, ${\mu }_{gly}=5\ $to $176\
\mathrm{cP}$, ${\rho }_{air}=1\ \mathrm{kg/m^{3}}$, $\mu
_{air}=0.017\ \mathrm{cP}$, ${\rho}_s=2650\ \mathrm{kg/m^3}$), the air-glycerin surface tension $\gamma =0.063\
\mathrm{kg/s^{2}}$, and the sand grain radius $r_s=100
\ \mu \mathrm{m}$. To mimic the existence of sub-REV scale heterogeneity, the solid fraction was initialized as a normally-distributed field ${\phi}_s=0.64 \pm
0.05$. To account for the non-reversible and compressive nature of the experiments,
the deformable solid was modeled as a Hershel-Bulkley-Quemada plastic with yield stress $\tau
_{yield}=16.02 \ \mathrm{m^{2}/s^{2}}$ \citep{Abou-Sayed2004,VanDam2002,Carrillo2020MDBB}. Permeability was
modeled as a function of porosity through the Kozeny-Carman relation:
$k=k_0{\phi}^3_f{\phi}^{-2}_s$ with $k_0=6.7\times{10}^{-12}\ \mathrm{m^2}.$ Relative
permeabilities were calculated through the Van Genutchen model \citep{VanGenutchen1980} and capillary effects were assumed negligible.

The resulting simulations were implemented in OpenFOAM{\circledR} within a 500 by 500 grid with
constant flow boundary conditions at the inlet, zero-gradient flow conditions out the
outlet, and no-slip boundary conditions for solid displacement at all boundaries. To allow
for a proper comparison between 2-D simulations and 3-D experiments in a Hele-Shaw cell of
thickness $a$, an additional drag term ($12\mu
a^{-2}{\boldsymbol{U}}_f$) was included in the fluid momentum equation \citep{Ferrari2015}.

\begin{figure}[htb!]
\begin{center}
\includegraphics[width=0.8\textwidth]{figures/PRL/Hang.png}
\caption[Continuous transition from fluid imbibition to fracturing in a Hele-Shaw cell]{\label{fig:Huang_Frac} Continuous transition from fluid imbibition to fracturing in a Hele-Shaw cell. Experimental images (A, B, C) were taken from \citet{Huang2012a} and numerically replicated in this study using equivalent conditions (D, E, F). Black lines represent the advancing saturation front.}
\end{center}
\end{figure}

The similarities between our model and the experiments are evident: as the viscous forces imposed on the solid increase, so does the system’s propensity to exhibit fracturing as the primary flow mechanism. Minor microstructural differences between our simulations and the
experiments reflect the manner in which the continuum-scale solid rheology model approximates the solid's granular nature. It is clear, however, that both systems are controlled by the balance between viscous forces and solid rheology at the scale of interest \citep{Carrillo2020MDBB}. 

\subsection{Creation of Fracturing Phase Diagrams}

We now use the simulation methodology presented above to identify the general non-dimensional parameters that control the observed 
transitional behavior between invasion and fracturing. To do so, we systematically varied
the solid's porosity ($\phi_f$ = 0.4 to 0.8), plastic yield stress ($\tau_{yield}$
= $1.5$ to ${24\ \mathrm{m^2/s^2}}$), capillary entry pressure ($p_{c,0}$ = $100$
to $50,000\ \mathrm{Pa}$), and permeability ($k$ = $1\times10^{-13}$ and $5\times10^{-9} \
\mathrm{m^2}$) and the invading fluid's viscosity ($\mu_n$ = $0.5$ to $50\ \mathrm{cP}$) and injection rate ($\boldsymbol{U}_f$ = $1\times10^{-4}$ to $8\times10^{-2} \
\mathrm{m/s}$). The only notable differences from the previous experiments are that we now include capillary effects and
model drainage as opposed to imbibition (i.e., the injected glycerin is now non-wetting to the porous medium). A
representative sample of the more than 400 resulting simulations is presented in the phase
diagrams shown in Fig. \ref{fig:phase_diagrams}.  

\begin{figure}
\begin{center}
\includegraphics[width=1\textwidth]{figures/PRL/SquarePhase.png}
\caption[Phase diagrams describing the effects of varying permeability, plastic yield stress, fluid injection rate, and capillary entry pressure on the transition from fluid drainage to fracturing]{\label{fig:phase_diagrams} Phase diagrams describing the effects of varying permeability, plastic yield stress, fluid injection rate, and capillary entry pressure on the transition from fluid drainage to fracturing. All cases are at ${\phi }_s=0.60\pm 0.05$ and ${\mu }_{n}=5\ \mathrm{cP}$. The remaining parameters are case-specific and can be found in each figure's upper legend. The areas separated by thin blue lines highlight four deformation regimes referred to here as the uniform invasion, fracturing, viscous transition, and capillary transition regimes. The color scheme is the same as in Fig. \ref{fig:Huang_Frac}.}
\end{center}
\end{figure}

Overall, the results make intuitive sense. Figure
\ref{fig:phase_diagrams}A shows that, \textit{ceteris-paribus}, less
permeable solids are more prone to fracturing. This is due
to the fact that, given a constant flow rate, lower permeability solids experience greater drag forces. Our results also show that solids
with lower plastic yield stresses fracture more readily, as their solid structure cannot
withstand the effects of relatively large viscous or capillary forces. The y-axis behavior of
Fig. \ref{fig:phase_diagrams}B further shows that systems with higher entry pressures are more likely to
fracture, i.e., the capillary stresses can overwhelm the solid's yield stress, in agreement with grain scale simulations \citep{Jain2009}. Finally, Fig.
\ref{fig:phase_diagrams}B also shows that higher injection rates lead to more fracturing, as these
increase the viscous drag effects on the solid structure.   

\section{Formulation of Non-Dimensional Controlling Parameters}

The deformation regimes observed in the previous experiments can be
delineated by defining two simple non-dimensional parameters that quantify the balance
between viscous pressure drop, solid softness, and capillary entry pressure.

\begin{equation}\label{N_vis_cart}
    N_{vis}=\frac{\Delta p}{{\tau }_{yield}{\rho }_s}=\frac{{\mu }UL}{{k\tau }_{yield}{\rho }_s}\ \ \ \  \textrm{(Cartesian)}
\end{equation}

\begin{equation}\label{eq:N_vis_radial}
    N_{vis}=\frac{\Delta p}{{\tau }_{yield}{\rho }_s}=\frac{{\mu }U{r}_{in}}{k{\tau }_{yield}{\rho }_s}{\mathrm{ln} \left(\frac{r_{out}}{r_{in}}\right)}\ \ \ \  \textrm{(Radial)} 
\end{equation}

\begin{equation} \label{Eq:N_cap} 
N_{cap}=\frac{p_{c,0}}{{\tau }_{yield}{\rho }_s}=\frac{2\gamma }{r_{pore}{\tau }_{yield}{\rho }_s} 
\end{equation} 

Here, the viscous fracturing number ($N_{vis}$) represents the ratio between the viscous pressure drop and the solid's structural forces. It embodies the question: ``Does fluid flow generate enough friction to induce fracturing?'' As shown in Fig. \ref{fig:Final_phase}, the answer is ``No'' if $N_{vis}<1$ and ``Yes'' if $N_{vis}>1.$ This number is the continuum scale analog of the ``fracturing number'' presented by \citet{Holtzman2012a} for granular solids. It also explains the experimental finding by \citet{Zhou2010} that fracture initiation is only a function of pressure, irrespective of the injection fluid viscosity. Furthermore, it elucidates why increasing the injection rate and decreasing the permeability have similar effects in Fig. \ref{fig:phase_diagrams}.

Complementarily, the capillary fracturing number ($N_{cap}$) represents the ratio between the the capillary entry pressure and the solid's structural forces; it embodies the question: ``Does multiphase flow generate enough capillary stresses to fracture the solid?''. Figure \ref{fig:Final_phase} shows that when $N_{cap}<1$ drainage is the preferential flow mechanism and when $N_{cap}>1$ fracturing becomes the dominant phenomenon.

\begin{figure}[htb!]
\begin{center}
\includegraphics[width=0.8\textwidth]{figures/PRL/FinalSquare.png}
\caption[Fluid invasion and fracturing in plastic porous media as a function of the viscous fracturing number and the capillary fracturing number]{\label{fig:Final_phase} Fluid invasion and fracturing in plastic porous media as a function of the viscous fracturing number $N_{vis}$ and the capillary fracturing number $N_{cap}$. Green triangles denote uniform invasion, red diamonds denote the transitional field spaces, and blue circles denote pure fracturing.}
\end{center}
\end{figure}

This analysis yields the rudimentary conclusion that uniform drainage should occur if either of the fracturing numbers is greater than unity, as confirmed by our simulations. However, our simulations further demonstrate the existence of three distinct fracturing regimes (Figs. \ref{fig:phase_diagrams}-\ref{fig:Final_phase}). In the first regime, referred to here as the \textit{fracturing zone}, both fracturing numbers are greater than unity. This leads to fracturing of the porous solid with minimal capillary invasion. In the second regime, referred to here as the \textit{viscous transition} ($N_{vis}>1$ and $N_{cap}<1$), only the viscous stresses are sufficiently large to fracture the solid. This leads to the formation of relatively wide fractures enveloped and preceded by a non-uniform invasion front. Finally, in the third regime, referred to here as the \textit{capillary transition} ($N_{vis}<1$ and $N_{cap}>1$), only the capillary stresses are sufficiently large to fracture the solid. Given a constant injection rate, this leads to the formation of fractures preceded by an invasion front, as in the viscous transition regime, but with subtle differences. Notably, the saturation front is more uniform (because of the lower viscous stresses) and the solid exhibits less compaction and hence narrower fractures (capillary stresses are localized at the invasion front, whereas the viscous stresses are more broadly and increasingly distributed throughout the porous medium). Finally, we note that the crossover between each of the four regimes is continuous, meaning that systems with $N_{vis}\sim1$ or $N_{cap}\sim1$ can share elements of neighboring regimes. 

\section{Influence of Capillary Heterogeneity}

Finally, we note that the simulations presented above were carried out using the simplifying assumption that the capillary pressure-saturation relationship is uniform within the porous solid. To evaluate the impact of this simplification on the results shown in Figs. \ref{fig:phase_diagrams}-\ref{fig:Final_phase}, we carried out additional simulations for all four regimes with a non-uniform capillary entry pressure distribution based on the Leverett J-function, where $p_{c,0}=p_{c,0}^*(\phi_s/\phi_s^{avg})^n$, $p_{c,0}^*$ is the capillary pressure at $\phi_s=\phi_s^{avg}$, and $n>0$ is a sensitivity parameter. \citep{CLeverett,Li2015}. The results show that increasing the value of $n$ stimulates the creation of finger-like instabilities at the fluid invasion front and leads to increased nucleation of small fractures at said position. Simulation predictions are shown in Fig. \ref{fig:variable_pc}. Despite the additional complexity of the resulting fluid invasion and fracturing patterns, our results with $n>0$ are consistent with the overall phase diagram presented in Fig. \ref{fig:Final_phase}. The results at $n=0$ are therefore highlighted in this text due to the significantly greater simplicity of their fluid and solid distribution patterns.

\begin{figure}[htb!]
\begin{center}
\includegraphics[width=0.9\textwidth]{figures/PRL/heterogeniousPc.png}
\caption[ The influence of capillary pressure heterogeneity on the capillary transition regime]{\label{fig:variable_pc} The influence of capillary pressure heterogeneity on the capillary transition regime. Here, $n$ represents the sensitive parameter in the Leverett J-function analogue. The color scheme is the same as in Fig. \ref{fig:Huang_Frac}.}
\end{center}
\end{figure}

\section{Conclusions}

In this chapter, we used the Multiphase DBB modeling framework to create a comprehensive phase diagram that identifies two non-dimensional parameters that categorize the crossover between fluid drainage and fracturing as a function of wettability, solid deformability, and hydrodynamics. In short, fracturing can occur whenever there is a high enough viscous and/or capillary pressure drop to overcome the solid structural forces. Furthermore, we showed that when it comes to systems with multiple fluids, it is also necessary to consider the effects of surface tension, wettability, and pore size into this analysis, as these parameters also control the fluids' propensity to fracture or invade the permeable solid. Lastly, we identified the theoretical existence of two characteristic transition zones between fluid invasion and fracturing that stem from the interaction of said fracturing numbers.

==> frontmatter/authorlist.tex <==
\noindent The following authors contributed to all Chapters: Francisco J. Carrillo and Ian C. Bourg.

\noindent The following authors contributed to Chapter \ref{chp:hybridPhase}: Francisco J. Carrillo, Cyprien Soulaine, and Ian C. Bourg.
